Human-in-the-Loop Methods for Data-Driven and Reinforcement Learning Systems

Recent successes combine reinforcement learning algorithms and deep neural networks, despite reinforcement learning not being widely applied to robotics and real world scenarios. This can be attributed to the fact that current state-of-the-art, end-to-end reinforcement learning approaches still require thousands or millions of data samples to converge to a satisfactory policy and are subject to catastrophic failures during training. Conversely, in real world scenarios and after just a few data samples, humans are able to either provide demonstrations of the task, intervene to prevent catastrophic actions, or simply evaluate if the policy is performing correctly. This research investigates how to integrate these human interaction modalities to the reinforcement learning loop, increasing sample efficiency and enabling real-time reinforcement learning in robotics and real world scenarios. This novel theoretical foundation is called Cycle-of-Learning, a reference to how different human interaction modalities, namely, task demonstration, intervention, and evaluation, are cycled and combined to reinforcement learning algorithms. Results presented in this work show that the reward signal that is learned based upon human interaction accelerates the rate of learning of reinforcement learning algorithms and that learning from a combination of human demonstrations and interventions is faster and more sample efficient when compared to traditional supervised learning algorithms. Finally, Cycle-of-Learning develops an effective transition between policies learned using human demonstrations and interventions to reinforcement learning. The theoretical foundation developed by this research opens new research paths to human-agent teaming scenarios where autonomous agents are able to learn from human teammates and adapt to mission performance metrics in real-time and in real world scenarios.

==> data/appendices.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.  
%
%
%  Author: Sean Zachary Roberson
%  Version 3.17.09
%  Last Updated: 9/21/2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{appendices}
\titleformat{\chapter}{\centering\normalsize}{APPENDIX \thechapter}{0em}{\vskip .5\baselineskip\centering}
\renewcommand{\appendixname}{APPENDIX}

\input{data/appendix1}
\input{data/appendix2}

\end{appendices}

==> data/bibliography.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.
%
%  Author: Sean Zachary Roberson
%	 Version 3.16.09
%  Last updated 9/12/2016
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           REFERENCES 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\phantomsection
\addcontentsline{toc}{chapter}{REFERENCES}

\renewcommand{\bibname}{{\normalsize\rm REFERENCES}}

%\bibliographystyle{ieeetr}
\bibliography{data/myReference}

==> data/cdc19.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           CDC                             %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter{\uppercase {Safely Learning Flight Control Systems in Real-Time from Human Demonstrations and Interventions}}

\textcolor{red}{*** [TODO] ***: Summarize introduction below}

\section{Introduction}

Advancements in automated systems and their proliferation to many application spaces has motivated development of increasingly capable intelligent agents. 
The design and implementation of \textit{a priori} or analytical control laws can be intractable or prohibitively challenging for many of the capabilities that are desired from autonomous or intelligent systems. 
Even in moderately complex scenarios, it can be infeasible to sufficiently understand and characterize the relevant system dynamics, including identification of system states and measurements, to enable design of effective controllers. 
In these cases, learning methods can provide a useful alternative to formulating a controller (often referred to as a \textit{policy}, with an \textit{agent} executing the policy in the environment) which maps observations of the state to actions. 
These learning methods do not allow for the analytical guarantees of controllability, observability, optimality, or even stability that can be derived from control theory. 
However, these techniques can produce highly effective policies to perform challenging tasks with relatively minimal first-principles design or tuning, even on embodied hardware platforms \cite{Ng2006,Ross2013,Giusti2015,Zhang2016,Bojarski2016,Gandhi2017,Goecks2018}.

Learning methods based on deep neural networks have demonstrated remarkable capabilities, from learning rich representations in computer vision tasks to automatic speech recognition and real-time translation \cite{LeCun2015, Schmidhuber2015, Hinton2012}.
Because of this success, there has been a growing interest in applying these techniques to learning optimal controllers for applications such as robotic grasping of objects, both in simulation \cite{Gu2017ICRA, Nair2018ICRA} and in physical robots \cite{OpenAI2018, Tobin2018IROS}, for robotic assembly \cite{Thomas2018ICRA} and for quad-rotor navigation and obstacle avoidance \cite{Blukis18, Anderson2018, Mei2016AAAI, Misra2017EMNLP, Tai2017IROS}.

This powerful, data driven approach to control optimization through self-learning requires large amounts of data (typically generated in a simulated software environment), and therefore lengthy training time, to converge when guided only by random exploration and feedback from the reward function. 
In addition, this method of learning can converge to policies that exploit idiosyncratic features of either the reward function or the simulator itself to produce undesirable behaviors. 
Also, implementation of poorly performing controllers prior to successful convergence risks catastrophic actions, which may not be tolerable on physical systems. 
Inputs from human users or observers can be utilized, through human-in-the-loop learning, to mitigate these drawbacks in several ways. 
For example, human interactions can be used as exemplar demonstrations of desired behavior \cite{Ross2013}, to preemptively intercede in avoiding catastrophic failure \cite{Hilleli2018}, or to indirectly guide learning through sparse evaluative feedback \cite{Warnell2018}. 
These modalities of interaction can focus learning, provide a measure of safety or boundedness in exploration, and encode intended behavior in the learning agent with efficient use of human effort.

This work focuses on the implementation of the first two stages of a framework that combines these various human interaction modalities to safely and efficiently train deep learning agent policies on a small unmanned aircraft system (sUAS), denoted as the Cycle-of-Learning (CoL) for Autonomous Systems from Human Interaction and detailed further in \cite{Waytowich2018,Goecks2019}. 
The first two stages of this framework comprise Learning from Demonstration (LfD) and Learning from Intervention (LfI), as shown in Fig. \ref{f:col_diagram2_colorblind}, which respectively allow a human to provide exemplar behaviors for the agent to imitate and to intercede preemptively when the agent is entering undesirable or potentially catastrophic states, generating corrective actions.
The two subsequent stages comprise Learning from Evaluation (LfE) and Reinforcement Learning (RL), not currently implemented in this work, but which respectively use human critiques of agent behavior to approximate a reward function and then leverage that human-derived reward function to optimize through recursive self-learning.

%% NW TODO: add a concluding paragraph to the intro to describe our results and contributions. 
In this paper, we apply the Cycle-of-Learning to a physical sUAS platform using a commercial Y6 hexrotor from 3DR (Berkeley, CA) and demonstrate its effectiveness in learning a control policy for an autonomous perching task.
We show that using this human-in-the-loop learning framework we can learn human-like control policies with minimal training time and achieve a similar task performance compared to standard control methods without any hand-tuning or first-principles design. 


\begin{figure}[thpb]
  \centering
  \includegraphics[width=\columnwidth]{col_diagram2_colorblind}
  \caption{Conceptual diagram of the Cycle-of-Learning for Autonomous Systems from Human Interaction. This work focuses on the first two stages of the cycle (dashed box).}
  \label{f:col_diagram2_colorblind}
\end{figure}

%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\section{Background}
% \subsection{Learning from Demonstrations and Interventions}
Deep neural networks fall under a class of learning methods called \textit{representation learning} \cite{LeCun2015} methods that allow a machine to learn from raw data and to automatically discover the feature representations needed for detection or classification. 
These methods learn multiple levels of feature representations with simple but non-linear modules that progressively transform the representation to higher levels of abstraction. 
Very complex functions can be learned as the depth (often referred to as the number of layers in the neural network) increases. 
This approach has been applied together with reinforcement learning (called deep reinforcement learning) to learn controllers that optimize an objective function or reward received through repeated interaction with an environment; for example, using deep reinforcement learning to solve for a controller that maximizes the game score in Atari games \cite{Mnih2015a}. 

Although deep neural network techniques have shown great success, they often require large amounts of data and lengthy training times to converge to good solutions.
Human-in-the-loop learning is a class of techniques that augment the learning process with human knowledge. 
\emph{Learning from Demonstration} is among the most common type of human-in-the-loop learning, which leverages human demonstrations or examples of the task for learning. 
A more comprehensive review of LfD can be found in \cite{Argall2009}; here we provide a brief summary of this technique, which is sometimes referred to as Imitation Learning or Behavioral Cloning.
In LfD, the policy $\pi_\theta$ is a function, parameterized by $\theta$, that maps from states $\vecb{s}$ to actions $\vecb{a}$.
\begin{equation} \label{eq:policy}
\pi_\theta : S \rightarrow A
\end{equation}
In control theory notation, $\vecb{s}$ would be analogous to the system state vector $\vecb{x}$, and $\vecb{a}$ would correspond to the control vector $\vecb{u}$ (Fig. \ref{f:blk_diag}a-b).
For the case of partial observability, observation $\vecb{o}$ would be used in place of state $\vecb{s}$, corresponding to the measurement vector $\vecb{y}$ used in control theory for systems without full-state feedback.

\begin{figure}[thpb]
  \centering
  \includegraphics[width=\columnwidth]{blk_diag}
  \caption{Block diagrams for a) typical feedback control systems and b) analogous learning agent systems with reward signal (dotted) in the case of RL. c) Inset diagram of the \emph{Agent} block for LfD and LfI, where the human triggers (dashed) switching between actions output by the current policy (black) and actions output from themselves with simultaneous policy update (gray).}
  \label{f:blk_diag}
\end{figure}

The policy $\pi_\theta$ is trained so as to generalize over a set $\mathcal{D}$ of states and actions visited during a task demonstration spanning $T$ time steps, i.e. a time history of state and action trajectories:
\begin{equation} \label{eq:demonstration_dataset}
\mathcal{D} = \left\{\vecb{a}_1, \vecb{s}_1, \vecb{a}_2, \vecb{s}_2, ... , \vecb{a}_T, \vecb{s}_T\right\}.
\end{equation}
This demonstration may be performed by an analytically derived controller, a pre-trained policy, or a human supervisor.
For example, \cite{Gandhi2017} designed a state machine controller to generate flight trajectories on a sUAS and to automatically label images based on collisions with objects in a cluttered environment.
The demonstrated trajectories were used to train a convolutional neural network (CNN) to perform reactive obstacle avoidance from monocular, forward-facing imagery when collisions were predicted to occur.

In the case of human demonstrations, the human provides the actions in response to observed states, subject to what may be represented as their internal policy $\pi_{sup}$, thereby generating $\mathcal{D}$. 
The training of policy $\pi_\theta$ therefore takes the form of a standard supervised learning problem to estimate the human's internal policy as $\hat{\pi}_{sup}$, where the parameters $\theta$ are trained in order to minimize a loss function, such as mean squared error, as shown in (\ref{eq:sup_mse}).

\begin{equation}\label{eq:sup_mse}
\hat{\pi}_{sup} = \argmin_{\pi_\theta} \frac{1}{T}\sum_{t=1}^{T} ||\pi_\theta(\vecb{s}_t) - \vecb{a}_t ||^2
\end{equation}

Several recent empirical successes have been demonstrated in applying imitation learning to train autonomous systems.
In the domain of self-driving cars, \cite{Bojarski2016} used human demonstrations to train a policy that mapped from front-facing camera images to steering wheel commands using approximately 100 hours of human driving data. 
Similar applications on sUAS have demonstrated navigation and obstacle avoidance through cluttered environments, using data collected from human users in various scenarios.
In \cite{Goecks2018}, a sparse number of human piloted trajectories were collected for sUAS flight through various high-fidelity cluttered simulation environments for training a controller to produce human-like velocity commands in response to depth imagery.
Real-world imagery was collected by \cite{Giusti2015} on three-camera sensor suite mounted to a human hiker through forest trails, to train a CNN for trail following sUAS control.
In \cite{Ross2013}, a sUAS was trained to avoid obstacles during flight using desired command inputs provided by a human observer in subsequent executions of the resultant policy, given a set of features derived from monocular camera imagery.

In \emph{Learning from Intervention} the human acts as a supervisor, observing the agent performing the task and intervening, that is overriding agent actions, when necessary to avoid undesirable or unsafe behaviors that may lead to catastrophic states. 
This technique was recently used to train agents without catastrophic failures, in a safe RL framework \cite{Saunders2017}. 
A human overseer monitored a learning agent and provided inputs that blocked the actions of the agent when the human deemed them to be potentially catastrophic, which were then used to train a function to perform this blocking automatically.
Similar work by \cite{Hilleli2018} used human interaction to train a classifier for detecting unsafe states.
This classifier was used to intervene in RL agent training, switching control from the current policy to a safe policy that was previously trained on human demonstration data, when an unsafe state was predicted. 
State-action trajectories generated by this intervening safe policy, considered \emph{off-policy} data as it was not produced by the current learning policy, were then combined with \emph{on-policy} data to re-train the learning agent, thereby improving its robustness.
These methods provide a measure of safety to agent training and boundedness to their exploration of the state space, which is critical for systems acting in the real world.

%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\section{Methodology}
This work demonstrates the hardware implementation of the Cycle-of-Learning, our recently developed technique for efficiently training an autonomous system safely and in real-time by combining LfD and LfI (Fig. \ref{f:col_diagram2_colorblind}), applied to a perching task on a multirotor sUAS. 
Successful demonstration of this human-in-the-loop learning algorithm in an analogous, though simulated, scenario is presented in \cite{Goecks2019}. 
In that work, human demonstrations and interventions were used to train a fully connected deep neural network to land a sUAS on a target landing pad in a high visual- and physical-fidelity drone simulator, Microsoft AirSim \cite{Airsim2017}.
The learned policy mapped inputs of vehicle inertial measurements and visual features of the target to velocity commands in the lateral, longitudinal, heave, and yaw degrees of freedom.
Training of the policy was performed in real-time and without any catastrophic actions, as they could be preemptively overridden by the human user.
The efficacy of the individual stages of LfD and LfI were compared against their partial sequencing, per the CoL framework, controlling for equivalent amounts of human interaction.
This demonstrated that the combination of these learning techniques in the CoL outperformed either technique in isolation and with greater data efficiency.

In this work, a very similar sensing, computational, and operational paradigm are implemented on a physical sUAS platform.
The CoL is initialized with a policy $\pi_\theta$ from a set of task demonstrations provided by the human trainer using a standard supervised learning technique.
Here, visual features of the perching target are extracted and concatenated with inertial measurements of the vehicle platform.
Simultaneous recording of the four-dimensional velocity commands are collected from the human user, via a joystick. 
Next, the agent is given control and executes $\pi_\theta$ while the human supervises the agent's actions. 
The human intervenes whenever the agent exhibits unwanted behavior, provides corrective actions, and then releases control back to the agent when they deem appropriate. 
The agent then learns from this intervention by augmenting the original training dataset with the states and actions recorded during the intervention, fine-tuning $\pi_\theta$. 
The agent executes the new policy $\pi_\theta$ as it is updated in real-time, with the human user continuing to supervise and intervene as needed, toggling control of the sUAS between themselves and the current agent policy via a button on the joystick.

The human user can fluidly switch at will between providing demonstrations, i.e. uninterrupted state-action trajectories for an entire landing maneuver, and interventions, i.e. corrective state-action trajectories applied to segments of the landing maneuver, (Fig. \ref{f:blk_diag}c).
By combining demonstrations and interventions, this framework can outperform a policy learned from human demonstrations alone, and with less training data. 
This effect is due in part to the more diverse exploration of the state space seen during the LfI stage than was experienced in the LfD stage, which would have resulted in failure. 
Targeted intervention during these failure states allows the agent to efficiently update the policy in its most deficient regions. 
The subsequent stages of the CoL, LfE and RL (Fig. \ref{f:col_diagram2_colorblind}), though not currently implemented would continue to optimize the policy as the agent becomes more proficient and autonomous.

%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\section{Experimental Setup}

The human operator switches at will between providing demonstrations and interventions by holding a trigger using a Xbox game pad (Firmware 2015) and has access to the live video feed from the onboard camera, as seen in Fig. \ref{f:col_human}. The perching task on a multirotor sUAS consists of using the onboard autopilot to command the vehicle to a random position in the xy-plane at a altitude of 1.5 meters. After take off, the goal is to land the vehicle on top of the landing marker based on the images returned by the camera, as seen in Fig. \ref{f:setup_mod}.

\begin{figure}[thpb]
  \centering
  \includegraphics[width=.95\columnwidth]{col_human_reduced}
  \caption{Interface between human operator and vehicle is given by a Xbox game pad and live video feed from the onboard camera.}
  \label{f:col_human}
\end{figure}

\begin{figure}[thpb]
  \centering
  \includegraphics[width=0.7\columnwidth]{setup_mod_reduced}
  \caption{Overview of the perching task. First, onboard autopilot commands takeoff to a random initial position. After reaching this initial point, the control is given to the learning agent policy to land the vehicle on top of the landing marker based on the images returned by the camera.}
  \label{f:setup_mod}
\end{figure}

The sUAS used to implement the learning framework is an adapted version of the commercial Y6 hexrotor from 3DR (Fig. \ref{f:hex_vehicle}). 
It uses a Pixhawk v1.0 as an autopilot and interfaces with the hexrotor actuators and onboard computer, an ODROID XU4 running Ubuntu 14.04.4 LTS. The vehicle is equipped with an ODROID camera with a resolution of 640x480 that streams data up to 12 Hz at flight time. 
The whole platform utilizes ROS Kinetic as the middle-ware allowing communication among autopilot, camera, control system, and joystick.
The position and orientation of the vehicle are recorded using a VICON Nexus 1.8.5 motion capture system.

\begin{figure}[thpb]
  \centering
  \includegraphics[width=\columnwidth]{hex_vehicle_reduced}
  \caption{Modified 3DR Y6 hexrotor with onboard camera, ODROID XU4, Pixhawk v1.0., and markers for the VICON motion capture system.}
  \label{f:hex_vehicle}
\end{figure}

A color segmentation computer vision (CV) algorithm extracts the x- and y-position of the fiducial landing target, a marker with a contrasting color when compared to the background, and its size (radius), which encodes distance to the target.
Measurements of 3D position, attitude (roll, pitch, and yaw), and estimated values of their velocities are provided by the VICON system.
The states $\vecb{s}$ are a concatenation of these twelve inertial states and the three visual features output by the CV algorithm.
The actions $\vecb{a}$ are the four joystick (roll, pitch, throttle, yaw) commands, which correspond to the velocity commands in the lateral, longitudinal, heave, and heading degrees of freedom.


The learning framework used in this work is summarized in Algorithm \ref{a:lfd_lfi}. 
The main procedure initializes the agent's policy $\pi_\theta$, the human dataset $\mathcal{D}$, and a secondary \emph{Policy Update} routine, which spawns a separate computational thread. 
The agent's policy $\pi_\theta$ is a fully-connected, three hidden-layer, neural network with 130, 72, and 40 neurons, respectively. 
The network is randomly initialized with weights sampled from a normal distribution. 
The state-action dataset $\mathcal{D}$ is initialized as an empty comma-separated value file.
The main loop primarily comprises reading the current agent-environment state and executing actions provided by either the agent's current policy or the human user.
When the human user interacts by holding a trigger on the joystick and providing input flight commands, these actions are executed by the agent and stored with the current state in the dataset $\mathcal{D}$.
This joystick trigger is used to toggle control authority between the human and the current policy, to prevent ambiguity or mistakenly interpreting only non-zero input commands as human-provided data.
If the human is not depressing this joystick trigger, actions $\vecb{a}$ are sampled from the current policy $\pi_\theta$, given the current state $\vecb{s}$, and executed by the agent.

In the secondary \emph{Policy Update} procedure, the loss threshold $l_{TH}$, the maximum number of training epochs $n_{max}$, and the batch size $N$ are initialized.
The procedure also spawns a separate computational thread to perform policy updates in real-time when the human user provides either demonstration or intervention data. 
This separate thread loads the current dataset $\mathcal{D}$ and continuously checks for newly added data, based on the number of samples.
If new samples are found, this loop samples a batch of $N=64$ state-action pairs from $\mathcal{D}$. 
Given these states $\vecb{s}$, corresponding actions $\hat{\vecb{a}}$ are sampled from the current policy $\pi_\theta$, and the mean squared error loss $l$ is computed:
\begin{equation}
    l = \frac{1}{N} \sum_{i=1}^{N} (\hat{\vecb{a}}_i - \vecb{a}_i)^2.
\end{equation}
If this loss is above the threshold $l_{TH}=0.005$ and the number of optimization epochs is below the maximum $n_{max}=2000$, the policy $\pi_\theta$ is optimized with the commonly used Root Mean Square Propagation (RMSProp) optimizer, with a learning rate of 1e-4.

For a comparative baseline, a classical proportional (P) feedback controller was also implemented to perform the landing task.
Given the relative simplicity of this task, the design problem is quite tractable.
Carefully tuning the gains of this system to generate desired landing behavior provides a benchmark of performance for our learning agent. 
The proportional controller (fixed gain P = 0.002) commands body-frame translational velocities in order to keep the vehicle in the center the landing marker in the image frame based on the estimated x and y coordinates extracted using the CV module. These commands are combined with a constant downward velocity of 0.024 m/s and no yaw control. The commanded velocities are translated to position and fed back based on VICON measurements. 


%% Cycle-of-Learning Pseudocode (updated)
\begin{algorithm}[!tb]
\caption{Cycle-of-Learning LfD and LfI Stages}\label{a:lfd_lfi}
\begin{algorithmic}[1]

\Procedure{Main}{}
    \Initialize{policy $\pi_\theta$, dataset $\mathcal{D}$}
    \Initialize{procedure \textsc{Policy Update}}
    % \State Define performance threshold $\alpha$
    \While {True}
        \State Record state $\vecb{s}$
        \If {Human interacting}
            \State Record human action $\vecb{a}$
            \State Add state-action pair $\vecb{s}$, $\vecb{a}$ to $\mathcal{D}$
        \Else
            \State Sample action $\vecb{a}$ from policy $\pi_\theta(\vecb{s})$
        \EndIf
        \State Execute action $\vecb{a}$
        \If {Task completed} %\If {End of episode}
            \State Reset state $\vecb{s}$
            \State \Return task completion reward $r$
        \EndIf
    \EndWhile
\EndProcedure

\Procedure{Policy Update}{}
    \Initialize{threshold $l_{TH}$, epochs $n_{max}$, batches $N$}
    \State Spawn separate thread
    \While {True}
        \State Load human dataset $\mathcal{D}$
        \If {New samples in $\mathcal{D}$}
            \While {$l > l_{TH}$ and $n < n_{max}$}
                \State Sample $N$ state-action pairs $\vecb{s}, \vecb{a}$ from $\mathcal{D}$
                \State Sample action $\hat{\vecb{a}}$ from policy $\pi_\theta(\vecb{s})$
                \State Compute loss $l$
                \State Increment epoch $n$
                \State Perform gradient descent update on $\pi_\theta$
            \EndWhile
        \EndIf
    \EndWhile
\EndProcedure

\end{algorithmic}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\section{Numerical Results}
%% TODOs for next version
% GG: In this plot, show the PID, human, and final policy of the CoL agent. In a separate plot, show the same data (position trajectories) for each successive episode of the CoL, using line type (dotted/solid) to indicate when control toggles between the human an policy. Color these in an ordinal manner (red-to-blue, or light gray-to-black) in their temporal sequence.}

% GG: Similar barplots to AAAI paper, but on hardware platform, illustrating performance and data efficiency between LfD, LfI, and CoL for only a few evaluations at most. Probably do not need results for multiple numbers of interaction, instead using whichever illustrates the point best.

% VL: once we get some human data, discuss how PID policy differs from human policy; i.e.: PID was less optimal/more noisy close to landing pad.

%Current results are preliminary and expected to be extended during the incoming weeks. At this stage, 
We compared trajectories generated by a human demonstrator and a controller designed using classic control theory. In addition, we also illustrate learning from interventions as the learning agent performs the task and the human operator corrects the behavior produced by the learned policy.

Humans naturally excel on vision-based tasks where noisy images, communication delay, occlusion, and lighting changes are present, tending to outperform CV approaches. Fig \ref{f:plot_pos} compares landing trajectories generated by a proportional controller and a human pilot for similar initial conditions. Fig. \ref{f:plot_vel} shows the linear velocities during these generated trajectories. Very close distances to the landing pad tend to increase noise in the CV module, which causes the performance of the proportional control to diminish, while the human performance remains more consistent throughout the task.

%% POSITION
\begin{figure}[thpb]
  \centering
  \includegraphics[width=1.0\columnwidth]{plot_pos}
  \caption{Comparison of vision-based landing trajectories generated by a proportional controller and human for similar initial conditions.}
  \label{f:plot_pos}
\end{figure}


%% VELOCITY
\begin{figure}[thpb]
  \centering
  \includegraphics[width=1.0\columnwidth]{plot_vel}
  \caption{Comparison linear velocities during vision-based landing trajectories generated by a proportional controller and human for similar initial conditions.}
  \label{f:plot_vel}
\end{figure}

To overcome these limitations, the Cycle-of-Learning (CoL) uses, in real-time, the trajectories demonstrated by the human as well as the partial trajectories demonstrated during the intervention phase. As the learning agent is trained in real-time, testing the performance can be done periodically on-the-fly. To evaluate the trained policy, the human operator gives control to the agent and observes the trajectories generated. In the event the controller performs an unexpected maneuver, the human intervenes and regains control. Figs. \ref{f:switch_pos} and \ref{f:switch_vel} shows the comparison of positions and linear velocities during a landing trajectory where the human intervenes to recover from a maneuver generated by the learning.

%% POSITION (SWITCH CASE)
\begin{figure}[thpb]
  \centering
  \includegraphics[width=1.0\columnwidth]{switch_pos}
  \caption{Comparison of positions during a landing trajectory where the human intervenes (Intervention) to recover from a maneuver generated by the learning agent using the Cycle-of-Learning (CoL).}
  \label{f:switch_pos}
\end{figure}


%% VELOCITY (SWITCH CASE)
\begin{figure}[thpb]
  \centering
  \includegraphics[width=1.0\columnwidth]{switch_vel}
  \caption{Comparison of linear velocities during a landing trajectory where the human intervenes (Intervention) to recovers from a maneuver generated by the learning agent using the Cycle-of-Learning (CoL).}
  \label{f:switch_vel}
\end{figure}

%In the incoming weeks more data will be collected and the controller will be evaluated and compared to classical approaches and human operator in terms of task completion, time to train, and amount of data required to learn a satisfactory controller in real-time.

% %% POSITION (INTERVENTION CASE)
% \begin{figure}[thpb]
%   \centering
%   \includegraphics[width=1.05\columnwidth]{interv_pos}
%   \caption{CAPTION.}
%   \label{f:interv_pos}
% \end{figure}


% %% VELOCITY (INTERVENTION CASE)
% \begin{figure}[thpb]
%   \centering
%   \includegraphics[width=1.05\columnwidth]{interv_vel}
%   \caption{CAPTION.}
%   \label{f:interv_vel}
% \end{figure}


%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\section{Summary}

%%%%%%%%%%%%%%%%%%%%
% \subsection{Conclusions}

In this work, we demonstrate the successful, safe, and efficient training of a deep learning agent to control targeted landing of a sUAS from human-provided demonstration and intervention data in real-time.
While this demonstrated landing behavior is fairly rudimentary and effectively solvable via traditional techniques of control theory, the algorithm and framework proposed here, the CoL, can allow for greater flexibility in learning new behaviors and abilities with less \emph{a priori} design and subsequent fine tuning.

%%%%%%%%%%%%%%%%%%%%
% \subsection{Future Works}

While we showed successful learning of flight controllers using relatively small amounts of human training data, our learning-based method requires our models to be trained or calibrated before the system can be used. Currently, this is done on hardware, however we would ideally like to train our flight controllers safely in simulation first, transfer the pre-trained controllers to hardware (such as in \cite{Sadeghi-RSS-17,Peng2018ICRA}) then fine-tune the controller with human interaction.
Additionally, having only implemented the first two stages of the CoL, future efforts will focus on integration of the remaining stages to improve the performance of the agent and demonstrate its ability to adapt to changing tasks and environmental factors.
We also aim to apply this framework to more challenging and complex tasks to highlight its unique capability of the CoL to imbue an embodied agent with intended behavior with limited design time and control tuning.

==> data/recommendations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.  
%
%
%  Author: Sean Zachary Roberson
%  Version 3.17.09
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           RECOMMENDATIONS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\chapter{RECOMMENDATIONS} \label{ch:recommendations}

Several recommendations are made based on the research in this dissertation:

\begin{enumerate}
    \item Investigate the trade-offs between learning in a simulated environment and transferring to hardware compared to directly learning in hardware. High-fidelity simulation environments take great effort and time to be implemented and there are no theoretical guarantees that the policy will be transferred successfully.
    \begin{itemize}
        \item How: As shown in this research with the Cycle-of-Learning and similar algorithms, as DAPG, if expert demonstrations are available, it is possible to integrate them to the reinforcement learning loop and learn directly in hardware. The time allocated to the development of the simulated environment can be shifted to collecting expert demonstrations.
    \end{itemize}
    \item Investigate the impact of neural network architecture size, mainly the number of hidden layers and neurons, on task performance when using machine learning algorithms, focusing on learning direct on hardware.
    \begin{itemize}
        \item How: Advances in the fields of Neural Architecture Search (NAS) and Neural Network Compression can be leverage to find smaller architectures with similar accuracy that can increase inference speed and allow complex models to be deployed on hardware.
    \end{itemize}
    \item Develop new algorithms focusing on realistic, and consequently more complex, scenarios, even at the cost of reduced performance. Although simple environments are important to develop and benchmark new algorithms, there is no theoretical guarantees that the performance will hold when they are applied to more realistic scenarios.
    \begin{itemize}
        \item How: When working with simulated environments, consider adding sensor noise, time synchronization, and high-fidelity dynamic models. Machine learning models are generally not robust to changes in the inputs distribution.
    \end{itemize}
    \item Consider the dynamic nature of human policies. This work assumed that the human policy remained fixed while training the learning agent and the human demonstrators were given practice time before performing the task. In reality, human performance can increase during training while the human learns to become better at performing the task or can degrade due to psychological factors.
    \begin{itemize}
        \item How: Add a confidence metric to the behavior cloning loss based on expertise of the human expert or current psychological states.
    \end{itemize}
    \item Investigate how to extend Cycle-of-Learning to teach a learning agent multiple tasks, as opposed to a single task as presented in this dissertation. This is essential to create learning agents that are able to fulfil additional roles in real-time tasks.
    \begin{itemize}
        \item How: Currently being developed by another graduate student in VSCL, Ritwik Bera, is a learning model that segments given demonstrations into differents options, which represent sub-tasks, and learns a option-conditioned policy.
    \end{itemize}

\end{enumerate}




==> data/section3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           METHODS                                %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter{\uppercase {Technical Approach - TODO: split between chapters}}

% ``The last invention that biological evolution needed to make - the neocortex - is inevitably leading to the last invention that humanity needs to make - truly intelligent machines.''

% - Ray Kurzweil, ``\textit{How to Create a Mind: The Secret of Human Thought Revealed}'', 2009 \cite{Kurzweil2012a}.

This section details the technical approach and theoretical foundations of the \nameProj (CoL). This section also details the proposed approach evaluation and how it compares to the current state-of-the-art RL algorithms.

%%% VGG: 10/22/2018
%%% EXTRA DETAILS OF COL
% \subsection{Data Efficiency}
% A demonstration is defined as a human-produced trajectory of state-action pairs for the entire episode, while an intervention is defined as a trajectory of state-action pairs for only the subset of the episode where corrective action is deemed necessary by the human. 
% Thus, the amount of data provided via intervention is nearly always less than the amount provided via demonstration. 
% %As episode length is not controlled for, it is possible for a intervention trajectory, resulting from a significant amount of corrective action, to result in more data than a more directed demonstration trajectory.
% Training routines that incorporate more episodes utilizing learning from intervention rather than learning from demonstration will in general be more data sparse, assuming comparable task performance.
% Therefore, by utilizing components of the CoL to learn from both demonstration and intervention, we can train with less data than if demonstrations had been used in isolation for an equivalent number of episodes, resulting in a more efficient training framework.
% This concept generalizes to the full CoL, as the agent naturally requires less input from the human as its policy develops, its task proficiency increases, and it becomes more autonomous (indicated in Figure \ref{fig:col_diagram}).

% \subsection{Safe Learning}
% The notion of \emph{safe} learning here refers to the ability of a human oracle to intervene in cases where catastrophic failure may be imminent.
% Thus, the agent is able to explore higher risk regions of the state space with a greater degree of safety.
% This approach leverages human domain knowledge and ability to forecast such boundary states, which the agent cannot do early in the training process when the state space is less explored.
% By allowing the policy to explore less seen regions and then provide training data of how to correct from those states, human interventions provide a richer dataset that improves the policy in those regimes.
% This is contrasted to a method based solely on demonstration, which may only see states and observations along a nominal trajectory and have a policy poorly fit to data outside that envelope.
% The result is a policy that is more robust, through greater data diversity, while not risking damage to the agent that is typical with methods that rely on random exploration of the state space.
% This provides a method to safely train an autonomous system.

% \subsection{Real-Time Interaction}
% The utility of the demonstrated approach is partially linked to the ability of the agent to consume data as it is provided by the human oracle and update its policy online.
% The current system accomplishes this by storing all subject state-action pairs in the training dataset, which is queried in real-time to update the policy, and then fine-tuning that policy whenever new samples are added to the dataset.
% During intervention, this allows for interaction with an agent using a policy trained on the most recent corrective actions provided by the human.
% The short time between novel human intervention data and behavioral roll-outs from the agent policy prevents significant delay in this feedback loop that might result from more infrequent, batch learning.
% As in closed loop systems, large temporal delays between feedback inputs and their resultant output behaviors can lead to instability.
% In this context, that would manifest as unstable training as the human oracle would need to correct for undesired actions for significantly longer before seeing any effect on the agent behavior.
% This shortcoming was exhibited in DAgger, where policy correction was a delayed, offline process.

\section{Preliminaries Concepts and Notation}

% Background on Reinforcement Learning (basic)
In \emph{Reinforcement Learning} (RL), it is desired to train an agent to learn the parameters $\theta$ of a \emph{policy} (or \emph{controller}) $\pi_{\theta}$, in order to map the partially-observable environment's \emph{observation} vector $\vec{o}$ (or \emph{state} vector $\vec{s}$ in fully-observable environments) to agent \emph{actions} $\vec{a}$. The performance of the agent is measured by a scalar \emph{reward signal} $r$ returned by the environment (external rewards, $r_e$) and/or returned by the agent itself (intrinsic rewards, $r_i$). At each time step $t$ the reward signal can be computed as the sum of all the extrinsic and intrinsic rewards received $r_t = r_{e_t} + r_{i_t}$. Figure \ref{fig:rl_classic} illustrates this description as a diagram. Mathematically, the RL problem is formalized as a \emph{Partially Observable Markov Decision Process} (POMDP) \cite{Bertsekas2000}. A POMDP $\mathcal{M} = \{ \mathcal{S},\mathcal{A},\mathcal{O},\mathcal{T}, r \}$ is characterize by its state-space $\mathcal{S}$ (where a vector of states $\vec{s} \in \mathcal{S}$), an observation-space $\mathcal{O}$ (where a vector of observations $\vec{o} \in \mathcal{O}$), an action-space $\mathcal{A}$ (where a vector of actions $\vec{a} \in \mathcal{A}$), a transition operator $\mathcal{T}$ (which defines the probability distribution $p(\vec{o}_{t+1}|\vec{o}_{t})$), and the reward function $r: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ (or $r(\vec{s},\vec{a}))$.

% Diagram RL
\begin{figure}[htbp]
    \centering
    \includegraphics[width=2.5in]{rl_classic}
    \caption{Reinforcement learning problem modeled as agent and environment interactions.}
    \label{fig:rl_classic}
\end{figure}

% This definition is illustrated by Equation \ref{eq:pomdp} and Figure \ref{f:pomdp}:

% \begin{equation} \label{eq:pomdp}
% \mathcal{M} = \{ \mathcal{S},\mathcal{A},\mathcal{O},\mathcal{T}, r \}.
% \end{equation}

% %SIMPLE POMDP
% \begin{figure}[!htb]%
%   \centering
%   \includegraphics[width=.5\linewidth]{simple_pomdp}%
%   \caption{Partially-Observable Markov Decision Process diagram \cite{DeepRLBerkeley2017}.}%
%   \label{f:pomdp}%
% \end{figure}

This interaction between agent and environment occurs during an \emph{episode}, which is defined as the time interval between the initial time step $t_0$ and the maximum number of time steps allowed $T$ or until a previously established metric is achieved. 
During an episode, the sequence of states observed and actions taken over a number of time steps $T$ can be represented by a \emph{trajectory} $\tau = \{ \vec{s}_0, \vec{a}_0, \vec{s}_1, \vec{a}_1, \ldots , \vec{s}_T, \vec{a}_T \}$.
The total reward per episode $R$ is defined as the sum of the rewards received for each time step, as shown in Equation \ref{eq:total_rew}.

\begin{equation}\label{eq:total_rew}
R = \sum_{t=0}^{T} r_t = \sum_{t=0}^{T} \left( r_{e_t} + r_{i_t} \right).
\end{equation}

Similarly, the expected total reward per episode received by a policy $\pi_\theta (\vec{a}_t | \vec{s}_t)$ can be defined by Equation \ref{eq:expected_rew}.

\begin{equation}\label{eq:expected_rew}
R_{\pi_\theta} = \sum_{t=0}^{T} \E_{\vec{a}_t \sim \pi_\theta} [r_t(\vec{s}_t, \vec{a}_t)].
\end{equation}

The probability of experiencing a given trajectory $\tau$ in a Markov Decision process can be written as
\begin{align}
\pi_{\theta}(\tau) &= p_{\theta} (\vec{s}_0, \vec{a}_0, \vec{s}_1, \vec{a}_1, \ldots , \vec{s}_T, \vec{a}_T) \\
&= p(\vec{s}_0) \prod_{t=0}^T \pi_{\theta}(\vec{a}_t|\vec{s}_t) p(\vec{s}_{t+1} | \vec{s}_t, \vec{a}_t).
\end{align}

The goal in RL is to find the parameters $\theta^*$ that will maximize the objective $J(\theta)$, which represents the expected total reward to be received by this policy $\pi_{\theta}(\tau)$.

As a side note, in Deep Reinforcement Learning (Deep RL), where deep neural networks are used as learning representation for the policies, a typical policy is represented by a neural network with two fully-connected layers with 64 neurons each (plus a bias term). If the dimension of the input is $N$ and the dimension of the output is $M$, this leads to $(N+1)*64 + (64+1)*64 + (64+1)*M$ parameters. For example, a policy for a continuous dynamical system with twelve inertial states and one control output would be represented by 5056 parameters.

To maximize $J(\theta)$, it is possible to compute its gradient with respect to its parameters $\theta$, as in Equations \ref{eq:j}, \ref{eq:j2}, and \ref{eq:grad_j}.

\begin{align} \label{eq:j}
J(\theta) &= \E_{\tau \sim p_{\theta} (\tau)} \left[ \sum_{t=0}^{T} r(\vec{s}_t, \vec{a}_t) \right]\\
&= \E_{\tau \sim \pi_{\theta} (\tau)} [r(\tau)] = \int(\pi_{\theta} (\tau) r(\tau) d\tau). \label{eq:j2}
\end{align}

\begin{equation} \label{eq:grad_j}
\nabla_{\theta} J(\theta) = \int(\nabla_{\theta} \pi_{\theta}(\tau) r(\tau) d\tau).
\end{equation}

% Using the following identity on Equation \ref{eq:grad_j}:

% \begin{equation} 
% \pi_{\theta}(\tau) \nabla_{\theta} \log \pi_{\theta}(\tau) = 
% \pi_{\theta}(\tau) \frac{\nabla_{\theta} \pi_{\theta}(\tau)}{\pi_{\theta}(\tau)} =
% \nabla_{\theta} \pi_{\theta}(\tau)
% \end{equation}

Equations \ref{eq:grad_j_id} and \ref{eq:grad_j_id2} are the result of using the identity $\pi_{\theta}(\tau) \nabla_{\theta} \log \pi_{\theta}(\tau) = 
\pi_{\theta}(\tau) \frac{\nabla_{\theta} \pi_{\theta}(\tau)}{\pi_{\theta}(\tau)} =
\nabla_{\theta} \pi_{\theta}(\tau)$ on Equation \ref{eq:grad_j}.

\begin{align} \label{eq:grad_j_id}
\nabla_{\theta} J(\theta) &= \int(\pi_{\theta}(\tau) \nabla_{\theta} \log \pi_{\theta}(\tau) r(\tau) d\tau)\\
&= \E_{\tau \sim \pi_{\theta} (\tau)} [\nabla_{\theta} \log \pi_{\theta}(\tau) r(\tau)]. \label{eq:grad_j_id2}
\end{align}

Reinforcement Learning is very closely related to the theory of classical optimal control, dynamic programming, stochastic programming, and optimization \cite{Powell2012}. However, while optimal control assumes perfect knowledge of the system's model, RL operates on measurements and reward function returned as consequence of interactions with an unknown environment \cite{Kober2015}.


% To simplify further derivation of the algorithm it is assumed a fully-observable environment, where the observation-space $\mathcal{O} = \mathcal{S}$ (state-space) and, consequently, vector of observations $\vec{o} = \vec{s}$ (states).

% At each time step $t$ of a finite time horizon $T$, the \emph{policy} (or controller) $\pi$, parametrized by $\theta_t$, maps the current environment's \emph{states} $\vec{s}_t$ to \emph{actions} $\vec{a}_t$: $\pi_{\theta}(\vec{a}_t|\vec{s}_t)$. This action affects the current environment's states $\vec{s}_t$ which evolves to $\vec{s}_{t+1}$ based on the environment's transition distribution (dynamics) $p(\vec{s}_{t+1}|\vec{s}_t,\vec{a}_t)$. The environment also returns a scalar \emph{reward function} $r$ that evaluates the action taken $\vec{a}_t$ at the state $\vec{s}_t$: $r(\vec{s}_t,\vec{a}_t)$.


% The probability of experiencing a given trajectory $\tau$ in a Markov Decision process can be written as:
% \begin{align}
% \pi_{\theta}(\tau) &= p_{\theta} (\vec{s}_0, \vec{a}_0, \vec{s}_1, \vec{a}_1, \ldots , \vec{s}_T, \vec{a}_T) \\
% &= p(\vec{s}_1) \prod_{t=1}^T \pi_{\theta}(\vec{a}_t|\vec{s}_t) p(\vec{s}_{t+1} | \vec{s}_t, \vec{a}_t)
% \end{align}

% The goal in RL is to find the parameters $\theta^*$ that will maximize the objective $J(\theta)$, which represents the expected total reward to be received by this policy $\pi_{\theta}(\tau)$:

% \begin{align}
% \theta^* &= \argmax_{\theta} J(\theta) \\
% &= \argmax_{\theta} \E_{\tau \sim p_{\theta} (\tau)} [\sum_{t=1}^{T} r(\vec{s}_t, \vec{a}_t)]
% \end{align}

% To maximize $J(\theta)$, it is possible to compute its gradient with respect to its parameters $\theta$:

% \begin{align}
% J(\theta) &= \E_{\tau \sim p_{\theta} (\tau)} [\sum_{t=1}^{T} r(\vec{s}_t, \vec{a}_t)]\\
% &= \E_{\tau \sim \pi_{\theta} (\tau)} [r(\tau)] = \int(\pi_{\theta} (\tau) r(\tau) d\tau)
% \end{align}

% Applying the gradient operator $\nabla_{\theta}$:

% \begin{equation} \label{eq:grad_j}
% \nabla_{\theta} J(\theta) = \int(\nabla_{\theta} \pi_{\theta}(\tau) r(\tau) d\tau)
% \end{equation}

% Using the following identity on Equation \ref{eq:grad_j}:

% \begin{equation} 
% \pi_{\theta}(\tau) \nabla_{\theta} \log \pi_{\theta}(\tau) = 
% \pi_{\theta}(\tau) \frac{\nabla_{\theta} \pi_{\theta}(\tau)}{\pi_{\theta}(\tau)} =
% \nabla_{\theta} \pi_{\theta}(\tau)
% \end{equation}

% \begin{equation}
% \nabla_{\theta} J(\theta) = \int(\pi_{\theta}(\tau) \nabla_{\theta} \log \pi_{\theta}(\tau) r(\tau) d\tau)
% \end{equation}

% \begin{equation} \label{eq:pg}
% \nabla_{\theta} J(\theta) = \E_{\tau \sim \pi_{\theta} (\tau)} [\nabla_{\theta} \log \pi_{\theta}(\tau) r(\tau)]
% \end{equation}

% Equation \ref{eq:pg} represents the \textbf{\emph{Policy Gradient}}.

% Substituting $\tau$ in terms of states and actions over time steps $t$ in a given time horizon $T$:

% \begin{equation} 
% \nabla_{\theta} J(\theta) = \E_{\tau \sim \pi_{\theta} (\tau)} [\sum_{t=1}^T \nabla_{\theta} \log \pi_{\theta}(\vec{a}_t | \vec{s}_t ) \sum_{t=1}^T r(\vec{a}_t, \vec{s}_t )]
% \end{equation}

Since the structure of the objective $J(\theta)$ and its gradient $\nabla_{\theta} J(\theta)$ are unknown, in practice the only way to evaluate them and approximate the expectation term is by sampling and averaging over $N$ samples:

\begin{equation}
\nabla_{\theta} J(\theta) \approx \frac{1}{N} \sum_{i=0}^N \left[ \left( \sum_{t=0}^T \nabla_{\theta} \log \pi_{\theta}(\vec{a}_t^{(i)} | \vec{s}_t^{(i)}) \right) \left( \sum_{t=0}^T r(\vec{a}_t^{(i)}, \vec{s}_t^{(i)}) \right) \right].
\end{equation}

% The policy is improved by \emph{gradient ascent} according to a step size $\alpha$, as shown in Equation \ref{eq:grad_ascent} and Figure \ref{fig:policy_imp}, optimizing the agent's policy during the training time.

% \begin{equation} \label{eq:grad_ascent}
% \theta \rightarrow \theta + \alpha \nabla_{\theta} J(\theta)
% \end{equation}

% \begin{figure}[!htb]%
%   \centering
%   \includegraphics[width=.45\linewidth]{policy_imp}%
%   \caption{Policy evaluation and optimization.}%
%   \label{fig:policy_imp}%
% \end{figure}


From a numerical optimization standpoint, as discussed in Section \ref{ssec:issues_rl}, it is infeasible to use this approach on large action- and observation-spaces (as it is the case for continuous robotics applications and vision-based tasks with images as input data) due to the low state-action pair visitation frequency, which reflects the  large number of samples required to correctly estimate the learning objective. On tasks with existing interaction between humans and intelligent agents, this research proposes using human input modalities to increase the sample-efficiency of reinforcement learning algorithms on large action and observation-spaces.


\subsection{Human Input Modalities}

% Human-in-the-loop approaches are ideal for vision-based learning tasks. The human visual cortex is a complex feature extractor with separate neural pathways to process different visual properties such as motion, depth, color, and shape. Humans are able to recognize objects with high accuracy and speed despite changes in lighting, resolution, motion, and other properties \cite{Grill-Spector2004}. This level of complexity and performance is difficulty to replicate on machines, but needed for advanced tasks.

Based on the cognitive neuroscience literature \cite{Gazzaniga2013}, there are direct and indirect ways to capture human-extracted features (i.e., response to a stimulus) and convert to digital signals, or \emph{human input modalities}, which can later be used on learning algorithms. Humans can be asked to perform the learning task and have their response logged (i.e., actions perform during the task through a joystick or where their eye gaze was focused using an eye tracking sensor) based on the stimulus presented (e.g., camera images); the logged demonstration data can be later used to train a \emph{behavior cloning} agent, which will replicate human behavior, or learn the cost function underlying the human behavior using \emph{inverse reinforcement learning} (IRL), as explained in more detail in the next sections. Humans can also \emph{intervene} while supervising a learning agent acting or \emph{evaluate} its behavior by converting this evaluation signal to a reward function. This iteration between demonstration, intervention, and evaluation, the core of the \emp{\nameProj} (CoL), has similarities to how humans teach each other.


\subsection{Inductive Bias}

% Definition
A core concept of learning is to be able to generalize from past experiences (for example, a training dataset) to address unseen situations \cite{mitchell1980need}.
Inductive bias refers to ``any basis for choosing one generalization over another, other than strict consistency with the observed training instances." \cite{mitchell1980need}.

% Importance
% How does it apply to this research proposal
This research work assumes that the human brain and its underlying decision process is nonlinear and stochastic. Nonlinear due to the neural pathway arrangement and connections \cite{Grill-Spector2004}, and stochastic in a sense that different action outputs can be observed from the same observation inputs depending on the current human emotional states \cite{de2006frames}.
To address this nonlinearity and stochasticity, this research adopts deep neural networks with Gaussian outputs to represent the learning policy.
This representation also allows processing the high-dimensional continuous observation and action-space encountered in real-world robotic applications.
By using neural networks it is also assumed that the policy to be learned, and the function that approximates it, has a smooth differentiable gradient which can be learned through back-propagation.
% How does it impact on the model selection (stop criteria during training)



%%% OLD DESCRIPTION FROM PREVIOUS PAPERS
% \subsubsection{Behavior Cloning} \label{sssec:behavior_cloning}

% \emph{Behavior Cloning}, or \emph{Imitation Learning}, is defined by training a policy $\pi$ in order to replicate an expert's behavior given states and actions visited during an expert demonstration
% \begin{align*}
% \mathcal{D} = \left\{\vec{a}_0, \vec{s}_0, \vec{a}_1, \vec{s}_1, ... , \vec{a}_T, \vec{s}_t\right\}.
% \end{align*}
% This demonstration can be performed by a human supervisor, optimal controller, or virtually any other pre-trained policy $\pi$. In the case of human demonstrations, the human expert is implicitly trying to maximize the reward function of a given task, as shown in Equation \ref{eq:imitation_rew}, where $\pi^*(\vec{a}^*_t | \vec{s}_t)$ represents the optimal policy (not necessarily known) in which the optimal action $\vec{a}^*$ is taken at state $\vec{s}$ for every time step $t$.

% \begin{equation}\label{eq:imitation_rew}
% \max_{\vec{a}_0,...,\vec{a}_T} \sum_{t=0}^{T} r_t(\vec{s}_t, \vec{a}_t) = \sum_{t=0}^{T} \log p (\vec{a}_t = \pi^*(\vec{s}_t) | \vec{s}_t)
% \end{equation}

% Defining the policy of the expert supervisor as $\pi_{sup}$ and its estimated policy as $\hat{\pi}_{sup}$, behavior cloning can be achieved through standard supervised learning (where the parameters $\theta$ of a policy $\pi_\theta$ are fit in order to minimize a loss function - such as mean squared error - as shown in Equation \ref{eq:sup_mse}) or using more advanced methods, such as Dataset Aggregation \cite{Ross2010} (DAgger, where data collected by the estimated policy is aggregated with data provided by the expert), Generative Adversarial Imitation Learning \cite{Ho2016} (where generative adversarial networks are used to fit distributions of states and actions defined by expert behavior), or Guided Cost Learning \cite{Finn2016} (where regularized neural networks and a cost learning algorithm based on policy optimization are used to learn the expert's cost function under unknown dynamics and high-dimensional continuous systems).


% \begin{equation}\label{eq:sup_mse}
% \hat{\pi}_{sup} = \argmin_{\pi_\theta} \sum_{t=0}^{T} ||\pi_\theta(\vec{s}_t) - \vec{a}_t ||^2
% \end{equation}


% \subsubsection{\textcolor{red}{TODO: }Inverse Reinforcement Learning} \label{sssec:irl}



% 1. CoL modeling and How prior knowledge is incorporated (human modalities)
\section{The \nameProj}

The \nameProj starts by randomly initializing an initial policy $\pi_0$, which could be represented as a neural network or any non-linear function approximation. With the policy initialized, a human trainer provides a set of task demonstrations while the sequence of observations $\vec{o}$ perceived (or states $\vec{s}$ extracted from these observations) and actions $\vec{a}$ taken are stored in a human dataset $\mathcal{D}_H$:

\begin{equation}
\mathcal{D}_H = \{ \vec{s}_0, \vec{a}_0, \vec{s}_1, \vec{a}_1, \ldots , \vec{s}_T, \vec{a}_T \}.
\end{equation}

In real-time, a sequence of previous human trajectories ($N$ state $\vec{s}_h$ and action $\vec{a}_H$ pairs) are uniformly sampled from $\mathcal{D}_H$. Given $\vec{s}_h$, actions $\vec{a}$ are sampled from the current policy $\pi$: $\vec{a} \sim \pi(\vec{s}_h)$. In order to \emph{learn from demonstrations}, \nameProj minimizes the L2-regularized mean square error loss $\mathcal{L}_D$ between human actions and actions sampled from the current policy, for all $K$ weights in the policy representation, where the strength of the regularization is controlled by the hyperparameter $\lambda$:

\begin{equation} \label{eq:mse_loss}
\mathcal{L}_D = \frac{1}{N} \sum_{i}^{N} (\vec{a}_H_i - \vec{a}_i)^2 + \frac{\lambda}{K} \sum_{k}^{K} w_k^2.
\end{equation}

The agent is still able to sample actions from the current policy $\pi$ while it is being trained. If at any time the agent exhibits unwanted behavior that diverges from the policy of the human trainer, the human is able to intervene and provide corrective actions to drive the agent back on course, and then releases control back to the agent. 
The agent then learns from this \emph{intervention} by augmenting $D_H$ with trajectories from the intervention, and updating the policy by minimizing the same loss function presented in Equation \ref{eq:mse_loss}. Figure \ref{fig:airsim_col_diagram_compact}  and Algorithm~\ref{alg:col_algo} illustrate the procedure in a scenario where a human trains an unmanned aerial system (UAS, quadrotor) to land on top of a vehicle (perching task).
It is important to notice that for the proposed research the policy is represented by a deep neural network, so there is no guarantee that the algorithm will converge to a local or global optimal policy in finite time. The main advantage of using deep neural networks is being able to approximate high-dimensional continuous observation and action-space encountered in mostly real-world robotic applications.

Combining demonstration and intervention data in this way should not only improve the policy over what learning from demonstration can do alone but also require less training data to do so. 
The intuition is that the agent will inevitably end up in states previously unexplored with the original demonstration data which will cause its policy to fail and that intervening from those failure states allows the agent to quickly learn from those deficiencies or ``blind spots'' in its own policy in a more targeted fashion than from demonstration data alone \cite{Ramakrishann2018}. 
In this way, learning occurs only from the critical states, which is more data efficient, instead of simply labeling all states taken from the agent, whether they be critical or not, by the human for training as is done in DAgger \cite{Ross2011}.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.75\linewidth]{airsim_col_diagram_compact3.png}
    \caption{Flow diagram illustrating the learning from demonstration and intervention stages in the \nameProj for the quadrotor perching task \cite{Goecks2019}.}
    \label{fig:airsim_col_diagram_compact}
\end{figure}

%% Cycle-of-Learning Pseudocode
\begin{algorithm}[!tb]
\caption{Combining Human Demonstrations and Interventions in the Cycle-of-Learning}\label{alg:col_algo}
\begin{algorithmic}[1]

\Procedure{Main}{}
    \State Initializes agent's policy $\pi$
    \State Initialize human dataset $\mathcal{D}_H$
    \State Initialize \emph{Update Policy} procedure (line \ref{alg_line:update_policy})
    \State Define performance threshold $\alpha$
    \While {task performance $< \alpha$}
        \State Read observation $o$
        \State Sample action $a_{\pi} \sim \pi$
        \If {Human Interaction ($a_H$)}:
            \State Perform human action $a_H$ from agent's policy \label{alg_line:agents_policy}
            \State Add $o$ and $a_H$ to $\mathcal{D}_H$
        \Else
            \State Perform $a_{\pi}$ 
        \EndIf
        \If {End of Episode}
            \State Evaluate task performance
        \EndIf
    \EndWhile
\EndProcedure

\Procedure{Update Policy}{} \label{alg_line:update_policy}
    \State Spawn separate thread
    \State Initialize $loss$ threshold $loss_{TH}$
    \While {\emph{Main} procedure running}
        \State Load human dataset $\mathcal{D}_H$
        \If {New Samples}:
            \While {$loss < loss_{TH}$ or $n$ epochs}
                \State Sample $N$ samples $o, a$ from $\mathcal{D}_H$
                \State Sample $\hat{a} \sim \pi$
                \State Compute $loss =
                \frac{1}{N} \sum_{i}^{N} (\vec{a}_H_i - \vec{a}_i)^2 + \frac{\lambda}{K} \sum_{k}^{K} w_k^2$
                \State Perform gradient descent update on $\pi$
                \State Update agent policy $\pi$ (line \ref{alg_line:agents_policy})
            \EndWhile
        \EndIf
    \EndWhile
\EndProcedure

\end{algorithmic}
\end{algorithm}


% As shown in Algorithm~\ref{alg:col_algo} the main procedure starts by initializing the agent's policy $\pi$, the human dataset $\mathcal{D}_H$, the \emph{Update Policy} subroutine, and task performance threshold. 
% The main loop consists of either executing actions provided by the agent or actions provided by the human. The agent reads an observation from the environment and an action is sampled based on the current policy. At any moment the human supervisor is able to override the agent's action by holding a joystick trigger. When this trigger is held, the actions performed by the human $a_h$ are sent to the vehicle to be executed and are added to the human dataset $\mathcal{D}_H$ to update the policy according to the \emph{Update Policy} subroutine.

% The agent's policy $\pi$ is a fully-connected, three hidden-layer, neural network with 130, 72, and 40 neurons, respectively. The network is randomly initialized with weights sampled from a normal distribution. The policy is optimized by minimizing the mean squared error loss using the Root Mean Square Propagation (RMSProp) optimizer with learning rate of 1e-4.
% Unless defined otherwise, the human dataset $\mathcal{D}_H$ is initialized as an empty comma-separated value (CSV) file. Its main goal is to store the observations and actions performed by the human.
% The procedure to update the policy in real-time spawns a separate CPU thread to perform policy updates in real-time while the human either demonstrates the task or intervenes. 
% This separate thread periodically checks for new demonstration or intervention data based on the size of the human dataset.
% If new samples are found, this thread samples a minibatch of 64 samples of observations and actions from the human dataset and is used to perform policy updates based on the mean squared error loss until it reaches the loss threshold of 0.005 or maximum number of epochs (in this case, 2000 epochs).
% This iterative update routine continues until the task performance threshold $\alpha$ is achieved, which can vary from task to task depending on the desired performance. For this work, we set $\alpha$ to 1 and only stop training after a pre-specified number of episodes defined in our experimentation methodology to empirically evaluate our method over a controlled number of human interactions, here defined as either human demonstrations or human interventions.

Demonstrations and interventions are able to shape the agent's behavior up to a certain point, but their policies are unable to adapt to changes in the environment unless new interventions are provided. This approach is sufficient for static scenarios but for the general case it is desired to optimize current performance metrics without constant human supervision.

An immediate approach would be to naively transfer the policy learned from demonstrations and interventions to a reinforcement learning algorithm for further optimization. Unfortunately, when using complex function approximation as learning representations (e.g. deep neural networks), the policy tends to be optimized to a local minima or saddle point where the policy gradient (on-policy) vanishes and utility functions converged to a sub-optimal value, halting further optimization after learning directly from demonstrations and interventions (off-policy). On-policy learning tends to be more stable (learns from the data currently being encountered by the policy), where off-policy tends to be more sample-efficient (can learn from previous data samples and multiple policies besides the one being followed).

\citeauthor{Gu2017} \cite{Gu2017} formalized the interpolation of on-policy policy gradient estimates with gradients of the estimate state-action function $\hat{Q}$ to compute the gradient of the performance metric to be optimized (Equation \ref{eq:ipg_grad}), where $\nu$ weights on-policy and off-policy gradients, $\rho_^\pi$ is the current policy sampling distribution, $\rho_^\beta$ is the off-policy sampling distribution, $\hat{A}$ is the estimated advantage function, and $Q^\pi_w$ is the off-policy estimated state-action function parametrized by $w$:

\begin{equation} \label{eq:ipg_grad}
    \nabla_\theta J(\theta) \approx (1-\nu) \E_{\rho^\pi,\pi}[\nabla_\theta \log \pi_\theta (a_t|s_t]) \hat{A} (s_t,a_t)] + \nu \E_{\rho^\beta} [\nabla_\theta \E_\pi [Q^\pi_w (s_t,.)]]. 
\end{equation}

The current state-of-the-art uses, as off-policy data, previous trajectories generated by the agent itself, prioritized by the temporal-difference error. Although effective, this approach does not encompass the exploration of regions of high return that are known to the human but not to the training agent.
Poor observation-space exploration leads to underestimation of the off-policy estimated state-action function $Q^\pi_w$, which contributes to the premature conversion of the estimated advantage function $\hat{A}$ to local minima.

This research proposes using human demonstrations and interventions directly to improve the estimation of the off-policy estimated state-action function $Q^\pi_H_w$ and the advantage function $\hat{A}_H$. Human demonstration and intervention trajectories stored in the dataset $D_H$ and sampled during each critic update to improve the estimates for $Q^\pi_H_w$ and for the expected discounted return $V_H$. Since the human explores regions of low and high return, $\hat{V}_H$ is more accurate than $\hat{V}$ estimated by the agent and, consequently, the advantage function, which is computed as $\hat{A}(s,a) = \hat{Q}(s,a) - \hat{V}(s)$, is better estimated by $\hat{A}(s,a) = \hat{Q}(s,a) - \hat{V}_H(s)$. Following the interpolation presented by \citeauthor{Gu2017} \cite{Gu2017}, the \nameProj uses the following cost gradient to update the agent's policy:

\begin{equation}
    \nabla_\theta J(\theta) \approx (1-\nu) \E_{\rho^\pi,\pi}[\nabla_\theta \log \pi_\theta (a_t|s_t]) \hat{A}_H (s_t,a_t)] + \nu \E_{\rho^\beta} [\nabla_\theta \E_\pi [Q^\pi_H_w (s_t,.)]].
\end{equation}


% 3. CoL Evaluation
\section{The \nameProj Evaluation}

\textbf{Validation: Experiments and Simulated Environment }
The \nameProj is tested (Figure~\ref{fig:airsim_col_diagram_compact}) in an autonomous quadrotor perching task using a high-fidelity drone simulator based on the Unreal Engine called AirSim developed by Microsoft \cite{Airsim2017}, as seen in Figure \ref{fig:Screenshot}. 
AirSim provides realistic emulation of quad-rotor vehicle dynamics while the Unreal Engine allows for the development of photo-realistic environments. The AirSim platform was chosen due to its high-fidelity physical and visual simulation, and for originally being designed for autonomous vehicles research and experimentation with deep learning, computer vision and reinforcement learning algorithms. This proposal refers the reader to the original paper \cite{Airsim2017} for more details about the architecture, simulation parameters, and accuracy of the model and flight characteristics when compared to a real quadrotor flying in real-world.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.75\linewidth]{Screenshot.png}
    \caption{Screenshot of AirSim environment and landing task. Inset image in lower right corner: downward-facing camera view used for extracting the position and radius of the landing pad which is part of the observation-space that the agent learns from. Video:\\ \url{https://youtu.be/1aktQxW7GQE}}
    \label{fig:Screenshot}
\end{figure}


The current observation-space consists of vehicle inertial and angular positions, linear and angular velocities, and pixel position and radius of the landing pad extracted using a hand-crafted computer vision module (15 dimensional continuous observation-space).
The vehicle is equipped with a downward-facing RGB camera that captures $320 \times 240$ pixel resolution images.  

The camera framerate and agent action frequency is \SI{10.5}{\hertz}, while the human observer views the video stream at approximately \SI{35}{\hertz}.  
The action-space comprises the four continuous joystick commands (roll, pitch, yaw, and throttle), which are translated to reference velocity commands (lateral, longitudinal, heading rate, and heave) by the vehicle autopilot. 

For the perching task, the goal is to land the quadrotor as close to the center of the landing pad as possible. Landing is successful if the quadrotor lands within \SI{0.5}{\meter} radius of the center of the platform and a failure otherwise. At the beginning of each episode, the quadrotor starts in a random x,y location at a fixed height above the landing pad and the episode ends when either the quadrotor reaches the ground (or landing pad) or after 500 time-steps have elapsed. 

% \textbf{Validation: Experiments and Simulated Environment }
% Aiming the development of novel techniques for human and intelligent agents interaction, one of the main interests of this project is the interaction between humans and unmanned air systems (UAS). The proposed approach is developed and tested using a simulated environment for the quadrotor flight and control.

% The Microsoft AirSim platform \cite{Airsim2017} is used as the virtual simulated environment. This platform simulates the quadrotor flight dynamics, onboard camera data (monocular RGB, ground truth depth, and random image segmentation), onboard inertial sensors (GPS, barometer, gyroscope, accelerometer, and magnetometer), collision, and environment interaction, as showed in Figure \ref{f:background:airsim_screen}.

% % AIRSIM SCREEN
% \begin{figure}[ht]
%  \centering
%  \includegraphics[width=.5\textwidth]{airsim_screen}
%  \caption{Microsoft AirSim sample screen displaying real-time onboard camera data: depth, image segmentation, and RGB view. Credits: \cite{Airsim2017}}
%  \label{f:background:airsim_screen}
% \end{figure}

\textbf{Verification: Performance Evaluation }
Using the AirSim landing task, the proposed \nameProj was tested against several baseline conditions where it was compared against using only a single human interaction modality (i.e. only demonstrations or only interventions) using equal amounts of human interaction time for each condition. By controlling for the human interaction time, it is possible to assess if utilizing multiple forms of human interaction provides an improvement over a single form of interaction given the same amount of human time. 

% Explain experimental protocol and evaluation
Each human participant (n=4, $\alpha$=0.1) followed the same experimental protocol: given an RGB video stream from the downward-facing camera, the participant controlled the continuous roll, pitch, yaw, and throttle of the vehicle using an Xbox One joystick to perform 4, 8, 12 and 20 complete episodes of the perching task for three experimental conditions: demonstrations only, interventions only, and demonstrations plus interventions with the CoL method, with each condition starting from a randomly initialized policy. For the CoL condition, participants performed an equal number of demonstrations and interventions to match the total number of episodes for that condition. 
For example, given 4 episodes of training, the CoL approach would train with learning from demonstrations in the first 2 episodes and then switch to learning from interventions for the last 2 episodes. 
The Col approach is compared to learning from demonstration for all 4 episodes as well as learning from interventions for all 4 episodes. 
This was repeated for 8, 12 and 20 episodes to study the effect of varying amounts of human interaction on task performance. 
Following the diagram in Figure \ref{fig:airsim_col_diagram_compact} and Update Policy procedure on Algorithm \ref{alg:col_algo}, the agent's policy is trained on a separate thread in real-time, and a model is saved for each complete episode together with the human-observed states and the actions they performed. 
These saved models are later evaluated for 100 tries to assess task performance.

The proposed research is also compared to a random agent and an agent trained using reinforcement learning. The reinforcement learning agent used Proximal Policy Optimization (PPO) \cite{Schulman2017}, the state-of-the-art policy gradient deep reinforcement learning algorithm, and was trained for 2500 episodes, using only task completion as a sparse binary reward signal. The sparse binary reward signal was chosen so the proposed approach could be applied to any task where it can be measure if the task was completed or not. The alternative solution would be to handcraft a specific reward function for each task, which would likely lead to better results (when compared to the sparse binary reward signal) but losing generality. Training time of the reinforcement learning agent was limited to the simulated environment running in real-time. 

% Performance of \nameProj is evaluated by comparison against standard well known RL algorithms: Deep Q-Networks (DQN) \cite{Mnih2013, Mnih2015} and Deep Deterministic Policy Gradient (DDPG)) \cite{Lillicrap2015a, Duan2016}; against well know human behavior cloning algorithm DAgger (Dataset Aggregation) \cite{Ross2010}; and against a human-level performance baseline.

% Algorithms are compared in terms of required time to achieve similar behavior, which is measured in terms of task-specific metrics. For the first task, it will be evaluate the average time to complete a given unseen obstacle avoidance task. Similarly for the second task, in which a performance metric can be constructed based on average time to localize the target.

% \section{Software Packages}
% The main software packages used during this research are Python \cite{Python} (general programming language), Numpy \cite{Numpy} (fundamental package for scientific computing with Python), Matplotlib \cite{Matplotlib} (plotting library for Python), TensorFlow \cite{Tensorflow} (interface for expressing machine learning algorithms), Keras \cite{Keras2015} (high-level library to interface with TensorFlow), OpenCV \cite{OpenCV} (image manipulation library), and Microsoft AirSim \cite{Airsim2017} (high-fidelity visual and vehicle dynamics simulation).

% 4. Comparison to the state-of-the-art
\section{Preliminary Results}

This section compiles preliminary results on different aspects of this proposed research.

%\subsection*{Human Input Modalities: Imitation Learning}
\textbf{Human Input Modalities: Imitation Learning}

This research proposes to increase the sample-efficiency of current RL algorithms by augmenting learning agents with human input modalities. One of the proposed human input modalities is demonstration of the task. Based on human demonstration of the task, the agent's policy is trained to minimize a loss function between the policy's suggested action and the action taken by the human, conditioned to the current observation. This leads to a policy that imitates human behavior. Human demonstration is used to overcome the initial exploration issue on RL problems, where random actions are taken in order to explore the state-space and its reward function structure.

Figure \ref{fig:bc_scenes} (link to videos) illustrates how human demonstration of the task is used to train a policy that is able to reproduce maneuvers performed by a human pilot to avoid obstacles in an indoor and outdoor simulated environment.

\begin{figure}[htb]%
    \centering
    \subfloat[Video (indoor warehouse environment): \url{https://youtu.be/Y2ceyDyg3AQ}]{{\includegraphics[width=.45\linewidth]{bc_scene0} }}%
    \qquad
    \subfloat[Video (outdoor forest environment): \url{https://youtu.be/rEbNytWz3c8}]{{\includegraphics[width=.45\linewidth]{bc_scene1} }}%
    \caption{Learning agents performing collision avoidance maneuvers based on demonstration provided by humans.}%
    \label{fig:bc_scenes}%
\end{figure}


\textbf{\nameProj Performance}

% Brief intro to results
%The Cycle-of-Learning methodology to combine human demonstrations and interventions is evaluated in terms of task completion  (during the evaluation phase, the percentage of episodes that the agent was able to complete the task: land the vehicle on top of the landing pad) and number of human data samples (observation-action pairs) used to train the model.


The \nameProj is evaluated in terms of task completion percentage, defined as the number of times the drone successfully landed on the landing pad over 100 evaluation runs, for each training method as well as for different amounts of human training data. Additionally, the \nameProj is evaluated based on the number of human data samples, i.e. observation-action pairs, used during training for each condition. 

%%%% PLOT PERFORMANCE
% Effectiveness (task completion) of the CoL when compared to imitation learning
\begin{figure}[t]
\centering
  \includegraphics[width=.65\linewidth]{figure4.pdf}
\caption{Performance comparison in terms of task completion with Interventions (Int), Demonstrations (Demo) and the Cycle-of-Learning (CoL) for (A) 4 human interactions, (B) 8 human interactions, (C) 12 human interactions and (D) 20 human interactions, respectively. Here, an interaction equates to a single demonstration or intervention and roughly corresponds to the number of episodes. Error bars denote 1 standard error of the mean.  The CoL outperforms Int and Demo across nearly all human interaction levels \cite{Goecks2019}.}
\label{fig:performance_all}
\end{figure}

%%%% PLOT NUMBER OF HUMAN SAMPLES
% Effectiveness (number of samples) of the CoL when compared to imitation learning
\begin{figure}[t]
\centering
  \includegraphics[width=.65\linewidth]{figure5.pdf}
\caption{Comparison of the number of human samples used for training with Interventions (Int), Demonstrations (Demo) and the Cycle-of-Learning (CoL) for (A) 4 human interactions, (B) 8 human interactions, (C) 12 human interactions and (D) 20 human interactions, respectively. Error bars denote 1 standard error of the mean. The CoL uses less data than the demonstration-only condition and only slightly more data than the intervention-only condition \cite{Goecks2019}.}
\label{fig:samples_all}
\end{figure}

Figure \ref{fig:performance_all} compares the performance of the models trained using only interventions (Int), the models trained using only demonstrations (Demo), and the models trained using the Cycle-of-Learning approach (CoL). 
Results are shown for only these conditions as the random policy condition and the RL condition trained using PPO were never successful. This can be attributed to the fact that in this task the agent commands four continuous actions and is rewarded only when the task is successful (binary sparse reward), which is unlikely to happen by only commanding random actions and, consequently, the agent never experiencing a useful policy gradient.
Barplots show the task completion performance from each condition averaged over all participants with error bars representing 1 standard error. 
Subpanels show the performance for varying amounts of human interaction: 4, 8, 12 and 20 episodes. The optimal number of human interactions (episodes) have not been investigate yet. The numbers were selected in order to constrain the time spent by the human performing the demonstrations and interventions.
For the 4 human interaction condition (Figure \ref{fig:performance_all}A), all methods show similar task completion conditions. 
However, for the 8, 12 and 20 human interaction conditions, the CoL approach achieves higher task completion percentages compared to the demonstration-only and intervention-only conditions, with the intervention condition performing the worst. 

For the final condition of 20 episodes the proposed approach achieves 90.25\% ($\pm$ 5.63\% std. error) task completion as compared to 76.25\% ($\pm$ 2.72\% std. error) task completion using only demonstrations (p=0.06651).
%In comparison, for the 8 episodes condition, the proposed approach achieves 74.75\% ($\pm$ 9.38\% std. error) task completion in contrast to 54.00\% ($\pm$ 8.95\% std. error) task completion when using only demonstrations. 


Figure \ref{fig:samples_all} compares the number of human data samples used to train the models for the same conditions and datasets as in Figure \ref{fig:performance_all}. 
For the final condition of 20 episodes the proposed approach used on average 1574.50 ($\pm$ 54.22 std. error) human-provided samples, which is 37.79\% fewer data samples when compared to using only demonstrations.
Note that the policies generated from this sparser dataset were able to increase task completion by 14.00\%. 
These results yield a CoL agent that has 1.90 times the rate of task completion performance per sample when compared to learning from demonstrations alone.
This value is computed by comparing the ratios of task completion rate to data samples utilized between the CoL agent and the demonstration-only agent, respectively. 
Averaging the results over all presented conditions and datasets, the task completion increased by 12.81\% ($\pm$ 3.61\% std. error) using 32.05\% ($\pm$ 3.25\% std. error) fewer human samples, which results in a CoL agent that overall has a task completion rate per sample 1.84 times higher than its counterparts.

Figure \ref{fig:ppo_curve} shows a comparison between the performance of the CoL method as well as the PPO baseline comparisons using a 2, 3 and 4 degree-of-freedom action space. For PPO with two actions, the agent was able to achieve 100\% task completion after 500 episodes, on average. However, when the action space complexity increases to three actions, the PPO agent performance was significantly reduced, now completing the task less than 5\% of the time after training for 1000 episodes. As expected, the PPO agent with the full four degree-of-freedom action space fails to complete the task after training for 1000 episodes. In contrast, the CoL method, with the same four degree-of-freedom action space, achieves about 90\% task completion in only 20 episodes, representing significant gains in sample efficiency compared to PPO.

%%%% PLOT PPO LEARNING CURVE
% \begin{figure}[t]
% \centering
%   \includegraphics[width=0.65\linewidth]{ppo_curve.png}
% \caption{Performance comparison between the Cycle-of-Learning (CoL) with four continuous actions and the Deep Reinforcement Learning algorithm Proximal Policy Optimization (PPO) trained for three different task complexities using 2, 3, and 4 continuous actions.}
% \label{fig:ppo_curve}
% \end{figure}

\begin{figure}[t]%
    \centering
    \subfloat[]{{\includegraphics[width=.46\linewidth]{ppo_curve.png} }}%
    \qquad
    \subfloat[]{{\includegraphics[width=.46\linewidth]{ppo_curve_log.png} }}%
    \caption{Performance comparison between the Cycle-of-Learning (CoL) with four continuous actions and the Deep Reinforcement Learning algorithm Proximal Policy Optimization (PPO) trained for three different task complexities using 2, 3, and 4 continuous actions. Same results in linear (a) and log scale (b) \cite{Goecks2019}.}
\label{fig:ppo_curve}
\end{figure}

\section{Discussion and Preliminary Conclusions}

%% Quick convergence and robust learning from CoL
Learning from demonstrations in combination with learning from interventions yields a more proficient policy based on less data, when compared to either approach in isolation.
The superior performance of the CoL is due to combining the two methods in sequence so as to leverage their strengths while attenuating their deficiencies.


Having been initialized to a random policy, learning from interventions alone produced more random behaviors, making convergence to a baseline behavior much slower.
Overall performance is thus slower to develop, resulting in lower percent completion for the same number of interaction episodes.
Conversely, learning from demonstrations alone was quicker to converge to stable behavior, but it was consistently outperformed by the CoL across varying numbers of interactions, while having more training data to utilize.
This seems initially counter-intuitive as more training data should result in a more accurate and presumably more proficient policy.
However, as the demonstrations typically follow stable trajectories, the agent is less likely to encounter regions of the state space outside these trajectories.
When enacting the policy at test time, any deviations from these previously observed states is not captured well in the policy, resulting in poor generalization performance.
By allowing the agent to act under its current policy, in conjunction with adaptively updating the policy with corrective human-provided actions needed to recover from potentially catastrophic states, the dataset and subsequent policy is improved.
Thus, the CoL allows for both rapid convergence to baseline stable behavior and then safe exploration of state space to make the policy more refined \emph{and} robust.
    
%% More data efficient
The results shown in Figure \ref{fig:samples_all} confirm the expectation that the combination of learning from demonstrations and interventions requires less data than the condition of learning from demonstrations alone, for the same number of episodes.
This supports the notion that the CoL is a more data efficient approach to training via human inputs.
When additionally considering the superior performance exhibited in Figure \ref{fig:performance_all}, the data efficiency provided by this technique is even more significant.
This result further supports the notion that a combinatorial learning strategy inherently samples more data rich inputs from the human observer.
 
It should be emphasized here that rather than providing an incremental improvement to a specific demonstration or intervention learning strategy, this work proposes an algorithmically agnostic methodology for combining modes of human-based learning that can be applied to any learning problem where human inputs can be collected.
%
Demonstrations and interventions ensure that the policy is trained more efficiently, learning at specific policy observation-space's blind spots, and leveraging human expertise to guarantee safety during training and learn without catastrophic failures. This approach bypasses the initial learning phase of traditional RL algorithms where failures are constant and performance is poorly, limiting their application to real-world robotic problems.
The evaluation phase is important to introduce a reward signal to the learning problem from a different human modality other than task demonstration and intervention.
%, or different from any reward signal that could have been previously designed.
This allows the agent to learn a reward function that can be used to guide RL algorithms at later stages of policy development.
The last phase, the RL phase, differently from pure RL, makes use of current data generated by the agent (on-policy data) and previous dataset (off-policy data) and policy built from human modalities, which is believed \cite{Gu2017} to guide the policy gradient updates to the same direction by interpolating on-policy and off-policy updates during the learning phase.
%
Preliminary results only account for the initial two modes of the CoL but the primary assertion of this work is that learning is made more robust, data efficient, and safe through a fluid and complementary cycling of these two modes, and would similarly be improved with the addition of the later stages of the CoL.

%Temporary subsection for clarity of organization but we'll remove later
\subsection{Current Limitations and Future Directions}

Preliminary results are limited to the first two stages of the CoL: learning from demonstrations and interventions.
Future work will include adding in more components of the CoL; for example:
\begin{enumerate}
    \item Learning from human evaluative feedback, as done in \cite{Knox2009,MacGlashan2017,Warnell2018}, and
    \item Reinforcement Learning techniques using an actor-critic style RL architecture \cite{Sutton1998} and interpolated policy gradient updates \cite{Gu2017}.
\end{enumerate}
%A second limitation of the current implementation is that it requires the human to supervise the actions taken by the agent at all times. 
%Future work aims to incorporate confidence metrics in our learning models so that the autonomous system can potentially halt its own actions when it determines it has low confidence and query the human directly for feedback in a mixed-initiative style framework \cite{Grollman2007}, similar to active learning techniques. 
Furthermore, preliminary results clearly indicate that a two-stage process --- with a primary stage with a large proportion of human-provided actions followed by a secondary stage with a smaller proportion of those actions --- outperforms processes with uniformly large or small amounts of human data throughout.

% Figure \ref{fig:performance_all} illustrates this notion across the varying number of interactions shown in the subfigures, i.e. through the change in relative performance between the three conditions.
% Rather than having a predetermined staging of the demonstrations and interventions that is potentially suboptimal, a mixed initiative framework could determine this optimal transition point.
% This could further reduce the burden on the human observer, allow for faster training, and even provide a mechanism to generate more robust policies through guided exploration of the state space.


